Deep Stacked Hierarchical Multi-patch Network for Image Deblurring

Despite deep end-to-end learning methods have shown their superiority in removing non-uniform motion blur, there still exist major challenges with the current multi-scale and scale-recurrent models: 1) Deconvolution/upsampling operations in the coarse-to-fine scheme result in expensive runtime; 2) Simply increasing the model depth with finer-scale levels cannot improve the quality of deblurring. To tackle the above problems, we present a deep hierarchical multi-patch network inspired by Spatial Pyramid Matching to deal with blurry images via a fine-to-coarse hierarchical representation. To deal with the performance saturation w.r.t. depth, we propose a stacked version of our multi-patch model. Our proposed basic multi-patch model achieves the state-of-the-art performance on the GoPro dataset while enjoying a 40x faster runtime compared to current multi-scale methods. With 30ms to process an image at 1280x720 resolution, it is the first real-time deep motion deblurring model for 720p images at 30fps. For stacked networks, significant improvements (over 1.2dB) are achieved on the GoPro dataset by increasing the network depth. Moreover, by varying the depth of the stacked model, one can adapt the performance and runtime of the same network for different application scenarios.

==> abstract.tex <==
\begin{abstract}
%In this paper, we address the problem of blind image deblurring for non-uniform motion blur. Conventional energy optimization-based methods fail to handle realistic non-uniform motion blur due to the underlying assumption of spatially-uniform blur. Recently, deep end-to-end learning  methods have shown their superiority in removing non-uniform motion blur. However, to achieve high-resolution and high-performance motion deblurring, most of these deep deblurring methods leverage multi-scale information, which makes the inference very expensive and far from real-time. In contrast to the multi-scale approaches, we propose a real-time high-performance motion deblurring approach that leverages local patch information. Specifically, we propose a simple but effective bottom-up deep image deblurring network which utilizes multiple image patches (fine-to-coarse extraction) as inputs. In this way, both the local and the global information are effectively integrated. Furthermore, to solve the problem that increasing depth with finer level can not improve the performance any more, we propose a effective stacking network, which can enhance the performance consistently with increasing the depth. Our proposed basic multi-patch unit achieves the state-of-the-art performance on the GoPro dataset while enjoying the fastest runtime. With 30ms to process an image at 1280$\times$720 resolution, our model runs at over 30fps, which makes it the first real-time deep motion deblurring model for 720p images. 

In this paper, we address the problem of blind image deblurring for non-uniform motion blur. Recently, deep end-to-end learning methods have shown their superiority in removing non-uniform motion blur. However, currently the multi-scale based deep models have two inherent problems: 1) very limited useful information can be learned via the multi-scale structure (less than 0.5dB performance improvement); 2) increasing the model's depth with finer scale level cannot increase the performance any more. To solve the efficiency problem, we present a deep multi-patch network that deals with blurry images from fine local regions. To tackle the depth problem, we propose an advanced stacking network based on our multi-patch model, whose performance can be improved by increasing depth very effectively. 
Our proposed basic multi-patch model achieves the state-of-the-art performance on the GoPro dataset while enjoying a 40$\times$ faster run time compared to current multi-scale methods. With 30ms to process an image at 1280$\times$720 resolution, it is the first real-time deep motion deblurring model for 720p images at 30fps. For stacking networks, impressive improvements (over 1.2dB) are observed on GoPro dataset by increasing the network depth. Varying depth of stacking model would affect the performance and run time meanwhile, thus satisfying the requirements in different scenarios.

%\YD{A dilemma: Are we presenting two approaches or one approach? How to highlight our proposed method? Efficiency or High Performance? Should we emphasize the original version or the stacked version? }

%Conventional energy optimization-based methods fail to handle realistic non-uniform motion blur due to the underlying spatially-uniform blur assumption. 

%Non-uniform blind image deblurring in dynamic scenes is a very challenging computer vision and image processing task. Conventional energy optimization based motion deblurring methods fail to address realistic non-uniform motion blur due to the underlying spatially-uniform motion blur assumption. Recently, end-to-end deep learning models have shown their superior ability in removing complex motion blurs. Most of the current deep deblurring methods focus on leveraging multi-scale information to restore sharp images. However, in this paper, we argue that leveraging the local information is also important. Many papers on fine-grained image classification have shown the benefit of aggregating over multiple locally extracted overlapping image patches. In this paper, we use the local information for deblurring which shows that complex non-uniform blurs can be removed more effectively. We propose a novel and effective bottom-up deep image deblurring network with multiple cropped image patches as inputs. Our experiments achieve the state-of-the-art on the GoPro dataset and demonstrate the superiority of our method. Moreover, our model enjoys the fastest runtime. With 30ms to process a 1280$\times$720 resolution image, this is the first real-time deblurring model for 720p images running at 30fps.
\end{abstract}

==> approach.tex <==
\section{Approach}
%\vspace{-0.2cm}
%\YD{We need to highlight the multi-patch structure and provide more insights and intuition. I will think about it and add it.}

By contrast to the expensive inference in multi-scale and scale-recurrent networks, we propose to exploit the multi-patch hierarchy. Our network is inspired by \cite{lazebnik2006beyond} which uses coarse-to-fine spatial pyramid matching for scene recognition as well as a classification pipeline \cite{koniusz2018deeper} which aggregates multiple image patches for better performance. We propose a novel deep hierarchical network based on multi-patch input. The differences between \cite{nah2017deep,tao2018scale} and our network are illustrated in Fig.~\ref{fig:Structure_Comp}. Despite our model uses a very simple architecture, it is very effective. To speed-up the runtime and reduce the complexity of training, skip and recurrent connections have not been used in our model. In contrast to \cite{nah2017deep} which uses upsampling links, we use much faster operations in our model such as concatenation, which is possible due to the multi-patch setup we employ. 


%=========================================================================
\subsection{Encoder-decoder Architecture}
Each level of our DMPHN network consists of one encoder and one decoder whose architecture is shown in Fig.~\ref{fig:encoder}.

Our encoder contains 15 convolutional layers, 6 residual links and 6 ReLU units. The layers of decoder and encoder are identical except that two convolutional layers are replaced by deconvolutional layers to generate images.

The parameters of our encoder and decoder are limited to 3.6MB. Our simple architecture %of encoder and decoder 
contributes to the fast deblurring runtime. By contrast, the multi-scale deblurring network in \cite{nah2017deep} has 303.6Mb parameters. 
%{\color{blue}Compared with our DMPHN models with 7.2 to 36.2MB parameters, }

\begin{figure}[tp]
\vspace{-0.3cm}
	\centering
	\includegraphics[width=8.5cm]{images/encoder-decoder}
	\caption{\small The structure of (a) decoder and (b) encoder.}
	\label{fig:encoder}
    \vspace{-0.3cm}
\end{figure}

\iffalse
\begin{figure*}[h]
	\centering
	\includegraphics[width=0.8\linewidth]{images/stack_model_sim.pdf}
	\caption{\small The network structure of Stack-DMPHN.}
	\label{fig:stack}
    \vspace{-0.3cm}
\end{figure*}

\begin{figure*}[tp]
	\centering
	\includegraphics[width=\linewidth]{images/v-stack_model_sim.pdf}
	\caption{\small The network structure of Stack-VMPHN.}
	\label{fig:v-stack}
    \vspace{-0.3cm}
\end{figure*}
\fi
\begin{figure*}[h]
	\centering
	\includegraphics[width=\linewidth]{images/stack_model_all.pdf}
	\caption{\small The network structure of stacking network. (a) Structure of Stack-DMPHN. (b) Structure of Stack-VMPHN. (c) The information flow of two stacking models. }
	\label{fig:stack}
    \vspace{-0.3cm}
\end{figure*}

%=========================================================================
\subsection{Network}
The architecture of our proposed DMPHN is shown in Fig.~\ref{fig:DMPHN}, in which we use the (1-2-4-8) model for illustration purposes.  
Notation (1-2-4-8) indicates the numbers of image patches from the coarsest to the finniest level \ie, a vertical split at the second level, $2\times 2 = 4$ splits at the third level, and $2\times 4 = 8$ splits at the fourth level.

We denote the initial blurry image input as ${\mathbf B}_1$, while ${\mathbf B}_{i，j}$ is the $j_{th}$ patch at the $i$-th level. Moreover, $f_i$ and $g_i$ are the encoder and decoder at level $i$, ${\mathbf C}_{ij}$ is the output of $f_i$ for ${\mathbf B}_{ij}$, and ${\mathbf S}_{ij}$ represents the output patches from $g_i$.

It can be seen that each level of our network consists of an encoder-decoder pair. The input for each level is generated by dividing the original input ${\mathbf B}_1$ into multiple non-overlapping patches. The output of both encoder and decoder from lower level (corresponds to finer grid) will be added to the upper level (one level above) so that the top level contains all learned information from finer levels. Note that the numbers of input and output patches at each level are different because the main idea of our work is for the lower level to focus on more local information (finer grid) to produce coarser gird (obtained by concatenating conv. features) which can be combined with the input of the next level (coarser grid). % because we concatenate the convolutional feature two by two in lower level to generate patches with the same size of the input at next upper level.

Taking the (1-2-4-8) structure as an example, the deblurring process of DMPHN starts from the bottom level 4. $B_1$ is sliced into $j\!=\!1,\cdots,8$ patches $B_{4j}$, which are fed into the encoder $f_i$ to produce convolutional feature representation:
\vspace{-0.1cm}
\begin{equation}
{\mathbf C}_{4j} = f_4({\mathbf B}_{4j}), \quad j\in\{1...8\}.
\end{equation}

Subsequently, we concatenate adjacent features to obtain new feature representation $C^*_{4j}$, which is of the same size as the convolutional feature representation at level 3.
\begin{equation}
{\mathbf C}^*_{4j} = \textrm{concat} ({\mathbf C}_{4,2j-1,}, {\mathbf C}_{4,2j}), \quad j\in\{1...4\}.
\end{equation}
%
The output of decoder $g_4$ is $S_{4j} = g_4({\mathbf C}^*_{4j})$. 

Next, we move one level up to level 3. The input of $f_3$ is updated to ${\mathbf B}_{3j} + {\mathbf S}_{4j}$. Once the output of $f_3$ is produced, we add to it  ${\mathbf C}^*_{4j}$:
\vspace{-0.1cm}
\begin{equation}
{\mathbf C}_{3j} = f_3({\mathbf B}_{3j} + {\mathbf S}_{4j}) + {\mathbf C}^*_{4j}, \quad j\in\{1...4\}.
\end{equation}

Again, we concatenate feature representation of level 3 to obtain ${\mathbf C}^*_{3j}$ and pass it through $g_3$ to obtain ${\mathbf S}_{3j}$:
\begin{align}
&{\mathbf C}^*_{3j} = \textrm{concat} ({\mathbf C}_{3,2j-1}, {\mathbf C}_{3,2j}), \quad j\in\{1, 2\},\\
%\end{equation}
%\vspace{-0.1cm}
%\begin{equation}
& {\mathbf S}_{3j} = g_3({\mathbf C}^*_{3j}), \quad j\in\{1,2\}.
\end{align}

Below we arrive at level 2 of our network which takes two image patches ${\mathbf B}_{21}$ and ${\mathbf B}_{22}$ as input. We update ${\mathbf B}_{2j}$ so that ${\mathbf B}_{2j}\!:=\!{\mathbf B}_{2j} + {\mathbf S}_{3j}$ and pass it through $f_2$:
\vspace{-0.1cm}
\begin{align}
&{\mathbf C}_{2j} = f_2({\mathbf B}_{2j} + {\mathbf S}_{3j}) + {\mathbf C}^*_{3j}, \quad j\in \{1,2\},\\
&{\mathbf C}^*_2 = \textrm{concat}({\mathbf C}_{21}, {\mathbf C}_{22}).
\end{align}

The residual map generated at level 2 is given by:
\vspace{-0.1cm}
\begin{equation}
{\mathbf S}_2 = g_2({\mathbf C}^*_2).
\end{equation}

For level 1, we obtain the final deblurred image $S_1$ as:
\vspace{-0.1cm}
\begin{align}
&{\mathbf C}_1 = f_1({\mathbf B}_1 + {\mathbf S}_2) + {\mathbf C}^*_2,
&{\mathbf S}_1 = g_1({\mathbf C}_1).
\end{align}

Different with \cite{nah2017deep} that uses the Mean Square Error (MSE) loss at each level, we use MSE only at the output of level 1 of the proposed model. The loss function of DMPHN is written as:
\begin{equation}
{\mathcal L} = \textrm{MSE}({\mathbf S}_1, {\mathbf G}),
\end{equation}
%
where ${\mathbf G}$ denotes the ground-truth clean image.

This objective function helps our network work in the principle similar to residual models. We investigated the use of multi-level MSE loss to force the output of each level to be close to the ground truth. However, our experiments have shown that there is no performance gain of such a loss. This is mainly due to the hierarchical multi-patch structure of our network, where the network learns to capture different image statistics at different levels.

\begin{figure*}[h]
\vspace{-0.3cm}
	\centering
	\includegraphics[width=0.9\linewidth]{images/Comp1}
	\caption{\small Deblurring results. Red block contains the blurred subject, blur and green are the results for \cite{nah2017deep} and \cite{tao2018scale} respectively, yellow indicates our result. It can be seen, our method produces the best facial details.}
	\label{fig:Comp1}
    \vspace{-0.3cm}
\end{figure*}

%=========================================================================
\subsection{Stackable Multi-Patch Network}
It is observed that applying finer level can no longer improve the performance any bit in both multi-scale and multi-patch network. Inspired by human's life experience on multi-level supervision mechanism, e. g., the employee from upper levels will supervise the work done by his lower level in a well-organized company, we propose a novel stacking structure to optimize deblurring task. 

Instead of making the network deeper vertically (adding finer level into the model, which increases the difficulty for single worker), we propose to increase the depth horizontally (stacking multiple models), which employs multiple workers (DMPHN) hierarchically to solve deblurring problem. 

There are several ways to cascade the models, here we employ two simplified diagrams to demonstrate the working process. The first one, called Stack-DMPHN, stacks multiple 'bottom-top' DMPHNs in the way showing in Fig.~\ref{fig:stack}. It can be seen that the tail of model $i-1$ and the head of model $i$ are connected along the model sequence, which means the optimization of model $i$ will be based on the output of model $i-1$. All intermediate features of model $i-1$ are passed to model $i$. MSE constraint is applied at the output of every sub-model in Stawck-SMPHN.

Alternatively, we investigate to reverse the direction of information flow, and propose a stackable v-shape 'top-bottom-top' multi-patch hierarchical network (Statck-VMPHN). Compared to DMPHN, the VMPHN structure can improve the performance more effectively in our experiments. The network structure of Stack-VMPHN is shown in Fig.~\ref{fig:stack}. The same with Stack-DMPHN, we employ MSE constraints at the end of every sub-model in Stack-VMPHN. 

The VMPHN is build upon our basic DMPHN and it can be regarded as a reversed version of Stack(2)-DMPHN. In Stack-DMPHN, the deblurring processing starts at bottom level and ends at top-level, then the output of top-level will be forwarded to bottom level of next model, however, VMPHN begins to work from top-level and it will turns back to top-level when arrive at the bottom-level.

The objective function for both Stack-DMPHN and Stack-VMPHN is as following:
\begin{equation}
    {\mathcal L} = \sum\limit_{i=1}^N \textrm{MSE}({\mathbf S}_i, {\mathbf G}),
\end{equation}
where N is the number of sub-models in stacking network, ${\mathbf S}_i$ represents the output of sub-model $i$, ${\mathbf G}$ denotes the ground-truth sharp image. 

Our experiments illustrate that the two types of stackable networks could enhance the deblurring performance consistently and effectively. Though the stack networks are proposed upon DMPHN, we believe they should be universal frameworks and all other deep deblurring methods can be embedded in this way to continuously improve the performance. 

\subsection{Network Visualization}
We visualize our proposed DMPHN output in Fig.~\ref{fig:Comp3} to show the contribution of each component.

As alluded in the previous section, DMPHN works as a form of residual network, which means that the finer level contains finer but visually less important information compared to the upper level. Taking DMPHN (1-2-4-8) as an example, we illustrate the output ${\mathbf S}_i$ of each level in Fig.~\ref{fig:Comp3}. It is clear that the information contained in ${\mathbf S}_4$ is the finest one. The outputs become more detailed, sharper and richer in color as we move up in DMPHN level by level.

%Furthermore, we verify the behavior of DMPNH by ablating different levels of a fully trained DMPHN (1-2-4-8) to analyze the contribution of each level. As shown in Fig.~\ref{fig:Comp4}, if we disconnect level 4, the generated image is still sharp but it lacks significant color information. However, the quality of the restored image drops dramatically when disconnecting level 3 and 4. By looking at the distortions, it appears as the local information has been corrupted by such an ablation. As we further disconnect level 2, the quality of image drops sharply. The output produced this way is the poorest.
%{\color{red}{I would be more convinced if I could see that without level 4 and 3, and 2, the ability of local deblurring drops}}

%In the above experiment, we have demonstrated that different levels of our DMPHN network contribute differently to the final restoration. The upper level generally contains more information but lower levels can deal locally with blur. 

\begin{figure}[h]
	\vspace{-0.3cm}
	\centering
	\includegraphics[width=\linewidth]{images/dmphn_comp.png}
    \caption{\small The outputs ${\mathbf S}_i$ for different levels of DMHPN(1-2-4-8). Four images from right to left are bottom level ${\mathbf S}_4$ to top level ${\mathbf S}_4$.}
	\label{fig:dmphn_comp}
    \vspace{-0.3cm}
\end{figure}

For stacked model, it is expected that the output of every sub-model is optimized level by level, which means the first output has the poorest quality and the last output achieves the best performance. Here we present the outputs of Stack(3)-DMPHN and Stack(3)-VMPHN to demonstrate both the two types of networks are working in the expected mode.
\begin{figure}[h]
	\vspace{-0.3cm}
	\centering
	\includegraphics[width=\linewidth]{images/sdnet_comp.png}
    \caption{\small The outputs for different sub-models of Stack(3)-DMHPN. From left to right are the outputs of $\mathbf{M}_1$ to $\mathbf{M}_3$.}
	\label{fig:sdnet_comp}
    \vspace{-0.3cm}
\end{figure}

\begin{figure}[h]
	\vspace{-0.3cm}
	\centering
	\includegraphics[width=\linewidth]{images/svdnet_comp.png}
    \caption{\small The outputs for different sub-models of Stack(3)-VMHPN. From left to right are the outputs of $\mathbf{M}_1$ to $\mathbf{M}_3$.}
	\label{fig:svdnet_comp}
    \vspace{-0.3cm}
\end{figure}
%=========================================================================
\subsection{Implementation Details}
All our experiments are implemented by PyTorch and evaluated on a single NVIDIA Tesla P100 GPU. To train DMPHN, we randomly crop the image to $256\times256$ pixel size. Subsequently, the cropped image will be sliced into different numbers of patches and forwarded to the inputs of each level. The batch size is set to 6 during training. The Adam solver \cite{kingma2014adam} is used for network training. We train our models for 3000 epochs in total. The initial learning rate is 0.0001 and the decay rate is 0.1 per 1000 epochs. We normalize the image values to $[0, 1]$ range and shift by 0.5 to set the range of input and output to be $[-0.5, 0.5]$.

==> conclusion.tex <==
\vspace{-0.3cm}
\section{Conclusions}
In this paper, we address the challenging problem of non-uniform motion deblurring by exploiting local image patches. We propose an end-to-end deep multi-patch hierarchical deblurring network. Compared with existing deep deblurring frameworks, our model achieves the state-of-the-art performance (according to PSNR and SSIM) and is able to run at 30fps for 720p images. Our work provides an insight for subsequent deep deblurring works regarding a more effective deblurring model. In the future, we will extend our multi-patch hierarchy framework to other low-level vision tasks such as image denoising and super-resolution, for which using the local information to deal with varied quantities of noise seems also as a reasonable assumption. 


==> experiments.tex <==
\section{Experiments}
%In this section, we present the experimental evaluation of our method.

\begin{table}[h]
\makebox{\begin{tabular}{|l|c|c|c|c|}
\hline
Models & \small PSNR & \small SSIM & Size & \small Runtime\\ \hline
Sun \etal \cite{sun2015learning} & 24.64 & 0.8429 & 54.1 & {\small 1.2$\times10^4$} \\
Nah \etal \cite{nah2017deep} & 29.23 & 0.9162 & 303.6 & {\small 4.3$\times 10^3$}\\
Zhang \etal \cite{zhang2018dynamic} & 29.19 & 0.9306 & 37.1 & {\small 1.4$\times 10^3$}\\
Tao \etal \cite{tao2018scale} & 30.10 & 0.9323 & 33.6 & {\small 1.6$\times 10^3$}\\ \hline
\small DMPHN(1) & 28.70 &  0.9131 & 7.2 & 5\\
\small DMPHN(1-2) & 29.77 & 0.9286 & 14.5 & 9\\
\small DMPHN(1-1-1) & 28.11 & 0.9041 & 21.7 & 12\\
\small DMPHN(1-2-4) & 30.21 & 0.9345 & 21.7 & 17\\
\small DMPHN(1-4-16) & 29.15 & 0.9217 & 21.7 & 92\\
\small DMPHN(1-2-4-8) & \textbf{30.25} & \textbf{0.9351} & 29.0 & 30\\
\small DMPHN(1-2-4-8-16) & 29.87 & 0.9305 & 36.2 & 101 \\
\hline
Stack(2)-DMPHN & 30.71 & 0.9403 & 43.4 & 34\\
Stack(3)-DMPHN & 31.14 & 0,9448 & 65.1 & 51\\
Stack(4)-DMPHN & \textbf{31.20} & \textbf{0.9451} & 86.8 & 68 \\
\hline
VMPHN & 30.89 & 0.9418 & 43.4 & 128\\
Stack(2)-VMPHN & \textbf{31.50} & \textbf{0.9483} & 86.8 & 164 \\
\color{red}{Stack(3)-VMPHN} & 31.28 & 0.9459 & 130.2 & 208\\
\hline
\end{tabular}}
\caption{\small Quantitative analysis of our proposed model on the GoPro dataset \cite{nah2017deep}. \textbf{Size} is measured by MB, \textbf{Runtime} is measured by second.} %Notation 2$\times$2 indicates that level 2 consists of two subwindows, which divide the initial images vertically and horizontally. }
\label{tabel:PSNR}
\vspace{-0.3cm}
\end{table}

\iffalse
\begin{table}[h]
\centering
\makebox{\begin{tabular}{|l|c|c|}
\hline
Models & PSNR & SSIM \\ \hline
Sun \etal \cite{sun2015learning} & 24.64 & 0.8429 \\
Nah \etal \cite{nah2017deep} & 29.23 & 0.9162 \\
Zhang \etal \cite{zhang2018dynamic} & 29.19 & 0.9306\\
Tao \etal \cite{tao2018scale} & 30.10 & 0.9323 \\ \hline
DMPHN(1) & 28.70 &  0.9131\\
DMPHN(1-2) & 29.77 & 0.9286 \\
DMPHN(1-1-1) & 28.11 & 0.9041\\
DMPHN(1-2-4) & 30.21 & 0.9345\\
DMPHN(1-4-16) & 29.15 & 0.9217\\
DMPHN(1-2-4-8) & \textbf{30.25} & \textbf{0.9351} \\
DMPHN(1-2-4-8-16) & 29.87 & 0.9305 \\
\hline
Stack(2)-DMPHN & 30.71 & 0.9403 \\
Stack(3)-DMPHN & 31.14 & 0,9448 \\
Stack(4)-DMPHN & \textbf{31.20} & \textbf{0.9451} \\
\hline
VMPHN & 30.89 & 0.9418 \\
Stack(2)-VMPHN & \textbf{31.50} & \textbf{0.9483} \\
\color{red}{Stack(3)-VMPHN} & 31.28 & 0.9459 \\
\hline
\end{tabular}}
\caption{\small Quantitative analysis of our proposed model on the GoPro dataset \cite{nah2017deep}.} %Notation 2$\times$2 indicates that level 2 consists of two subwindows, which divide the initial images vertically and horizontally. }
\label{tabel:PSNR}
\vspace{-0.3cm}
\end{table}

\begin{table}[h]
\centering
\makebox{\begin{tabular}{|l|c|c|}
\hline
Models & Size (MB) & Runtime (ms)\\ \hline
Sun \etal \cite{sun2015learning} & 54.1 & 1200$\times10^3$\\
Nah \etal \cite{nah2017deep} & 303.6 & 4.3$\times10^3$ \\ 
Zhang \etal \cite{zhang2018dynamic} & 37.1 & 1.4$\times10^3$\\
Tao \etal \cite{tao2018scale} & 33.6 & 1.6$\times10^3$ \\ \hline
DMPHN(1) & 7.2 & 5\\
DMPHN(1-2) & 14.5 & 9\\
DMPHN(1-1-1) & 21.7 & 12 \\
DMPHN(1-2-4) & 21.7 & 17 \\
DMPHN(1-4-16) & 21.7 & 92\\
DMPHN(1-2-4-8) & 29.0 & 30\\
DMPHN(1-2-4-8-16) & 36.2 & 101 \\
\hline
Stack(2)-DMPHN & 43.4 & 34 \\
Stack(3)-DMPHN & 65.1 & 51 \\
Stack(4)-DMPHN & 86.8 & 68 \\
\hline
VMPHN & 43.4 & 128 \\
Stack(2)-VMPHN & 86.8 & 164 \\
Stack(3)-VMPHN & 130.2 & 208\\
\hline
\end{tabular}}
\caption{\small The size and runtime analysis of the proposed model on the GoPro dataset \cite{nah2017deep}. The reported time is the CNN runtime (the time of writing generated images to disk is not considered).}
\label{table:Size}
\end{table}
\fi

\subsection{Dataset}
We train and evaluate the proposed model on several different variants of the GoPro dataset \cite{nah2017deep}. The \textbf{GoPro} dataset \cite{nah2017deep} consists of 3214 pairs of blurred and clean images from 33 sequences captured at 720$\times$1280 resolution. The blurred images in this dataset are generated by averaging varying number (7--13) of successive latent frames to produce blurs of different strength. For a fair comparison, we follow the protocol in \cite{nah2017deep}, which uses 2103 image pairs for training and the remaining 1111 pairs for testing.

\textbf{VideoDeblurring} dataset proposed by \cite{su2017deep} contains videos captured by various devices, such as iPhone, GoPro and Nexus. The quantitative part has 71 videos and every video consists of 100 frames at 720$\times$1280 resolution. Following the setup in \cite{su2017deep}, we use 61 videos for training and the rest 10 videos for testing. In addition, we evaluate the model trained on GoPro dataset\cite{nah2017deep} on this dataset  to evaluate the generalized ability. %

%\noindent{\textbf{Synthetic dataset}} proposed in \cite{lai2016comparative} is generated by convolving different non-uniform kernels with the latent clean images. The blurred and clean images provided in this dataset are not aligned in the same way with GoPro dataset, which makes the quantitative analysis, \eg, Peak Signal-to-Noise Ratio (PSNR) and Structural Similarity (SSIM) \cite{wang2004SSIM} less correlated with the perceptual image quality. Thus, we present deblurred instances to demonstrate the performance rather than the quantitative results.

\begin{table}[h]
\centering
\makebox{\begin{tabular}{|l|c|c|c|}
\hline
Models & PSNR & SSIM & Runtime\\ \hline
Nah \etal \cite{nah2017deep} & 29.23 & 0.9162 & $1.4\times10^3$\\ \hline
DMSN(1) &  28.70 & 0.9131 & 4\\ 
DMPHN(1) &  28.70 & 0.9131 & 4\\ \hline
DMSN(2) &  28.82 & 0.9156 & 21\\
DMPHN(1-2) & 29.77 & 0.9286 & 9 \\ \hline
DMSN(3) &  28.97 &  0.9178 & 27\\
DMPHN(1-2-4) & 30.25 & 0.9351 & 17\\
\hline
\end{tabular}}
\caption{\small The baseline performance of multi-scale and multi-patch methods on the GoPro dataset \cite{nah2017deep}. Note that DMSN(1) is identical to DMPHN(1).} 
\label{tabel:PSNR_sc}
\end{table}

\begin{table}[h]
\centering
\makebox{\begin{tabular}{|l|c|c|c|}
\hline
Models & PSNR & SSIM & Size (MB)\\ \hline
DMPHN(1-2) & 29.77 & 0.9286 & 14.5\\
DMPHN(1-2)-WS & 29.22 & 0.9210 & 7.2\\
DMPHN(1-2-4) & 30.21 & 0.9343 & 21.7\\
DMPHN(1-2-4)-WS & 29.56 & 0.9257 & 7.2\\
DMPHN(1-2-4-8) & 30.25 & 0.9351 & 29.0\\
DMPHN(1-2-4-8)-WS & 30.04 & 0.9318 & 7.2\\ \hline
\end{tabular}}
\caption{\small Quantitative analysis of the weight sharing mechanism on the GoPro dataset \cite{nah2017deep}.}
\label{tabel:share_weight}
\vspace{-0.3cm}
\end{table}


\begin{table*}[ht]
\vspace{-0.3cm}
\centering
\makebox{\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Methods & Train & \#1 & \#2 & \#3 & \#4 & \#5 & \#6 & \#7 & \#8 & \#9 & \#10 & {\small Average} \\ \hline
Input & - & 24.14 & 30.52 & 28.38 & 27.31 & 22.60 & 29.31 & 27.74 & 23.86 & 30.59 & 26.98 & 27.14 \\
PS\small{Deblur} & - &24.42 & 28.77 & 25.15 & 27.77 & 22.02 & 25.74 & 26.11 & 19.75 & 26.48 & 24.62 & 25.08 \\
WFA \cite{delbracio2015hand} & Y & 25.89 & 32.33 & 28.97 & 28.36 & 23.99 & 31.09 & 28.58 & 24.78 & 31.30 & 28.20 & 28.35 \\
Su \etal \cite{su2017deep} & Y & 25.75 & 31.15 & 29.30 & 28.38 & 23.63 & 30.70 & 29.23 & 25.62 & 31.92 & 28.06 & 28.37 \\ \hline
Ours({\color{red} updating}) & N & 27.32 & 31.56 & 30.25 & 29.97 & 24.17 & 31.39 & 29.71 & 26.17 & 32.54 & 27.91 & 29.10 \\ 
Ours({\color{red} updating}) & Y & 29.32 & 33.54 & 31.66 & 31.18 & 26.05 & 32.65 & 30.45 & 27.12 & 34.72 & 29.92 & 30.74 \\ \hline
\end{tabular}}
\caption{\small Quantitative analysis (PSNR) on the VideoDeblurring dataset \cite{su2017deep} for models trained on GoPro dataset. PSDeblur means using Photoshop CC 2015. \textbf{Train} option denotes if the method has been trained on \textbf{VideoDeblurring} dataset. We select 'single frame' version of \cite{su2017deep} for fair comparison. }
\label{tabel:share_weight}
\vspace{-0.3cm}
\end{table*}

\subsection{Evaluation Setup and Results}
We feed the original high-resolution $720\times1280$ images into DMPHN for the performance analysis. The PSNR and SSIM are reported in Table \ref{tabel:PSNR}. In addition, we present the model size and runtime in Table \ref{table:Size} for an in-depth comparison with other state-of-the-art deblurring models. For Stack-models, we employ (1-2-4) structure as the basic model unit to reduce runtime as well as the difficulty of training.

%\subsection{Results}
\noindent{\textbf{Performance.}} From Table \ref{tabel:PSNR}, it can be seen that our proposed DMPHN outperforms other methods according to PSNR and SSIM, which demonstrates the superiority of non-uniform blur removal via the localized information our model uses. The deepest DMPHN we trained and evaluated is (1-2-4-8-16) due to the GPU memory limitation. The best performance is obtained with (1-2-4-8) model, for which PSNR and SSIM are higher compared to all current state-of-the-art models. Note that our model is simplifier than any other approaches as we do not apply any recurrent units in our network. We note that patches that are overly small (below 1/16 size) are not helpful in the motion blur removal.

The deblurred images from the GoPro dataset are shown in Fig. ~\ref{fig:Comp1} and \ref{fig:Comp2}. In Fig.~\ref{fig:Comp1}, we show the deblurring performance of different models for image containing heavy motion blur. We zoom on the main object for clarity. In Fig.~\ref{fig:Comp2}, we select the pictures of different scenes to demonstrate the advantages of our model. As can be seen, our DMPHN obtains the best detail representations in any cases.



\noindent\textbf{Runtime}. In addition to the good PSNR and SSIM results on our model, to the best of our knowledge, DMPHN is also the first deep deblurring model that can deblur images real-time. For example, DMPHN (1-2-4-8) takes 30ms to process a 720$\times$1280 image, which means it supports real-time 720p image deblurring at 30fps. However, there are runtime overheads related to I/O operations, so the real-time deblurring application requires fast transfers from video grabber to GPU, larger GPU memory and/or an SSD drive, \etc. 
%requires the supports of powerful large-memory GPU and SSD to accelerate this process.

There are several factors contributing to the fast runtime: (i) shallower encoder-decoder with a small convolutional kernel size; (ii) removal of unnecessary links \eg, skip and recurrent connections; (iii) avoiding upsampling and deconvolution operations \cite{long2015fully}. 

\noindent \textbf{Baseline Comparison.} Though our model has a much better performance than the multi-scale model \cite{nah2017deep}, it is an unfair comparison because the network structures of our proposed model and \cite{nah2017deep} differ significantly. Compared with \cite{nah2017deep}, which uses over 303.6MB parameters, we apply much shallower CNN encoders and decoders with the model size 10$\times$ smaller. Thus, we create a Deep Multi-Scale Network (DMSN) that uses our encoder-decoder following the setup in \cite{nah2017deep} for the baseline comparison (sanity check) between multi-patch and multi-scale methods. As Table \ref{tabel:PSNR_sc} shows, the PSNR of DMSN is worse than \cite{nah2017deep}, which is normal due to our simplified CNN architecture. Compared with our DMPHN, the best result obtained with DMSN is worse than the DMPHN(1-2) model. Due to the common testbed, we argue that the performance of DMSN and DMHPN reported by us is the fair comparison of the multi-patch hierarchical model and multi-scale model \cite{nah2017deep}.

\vspace{0.3cm}
\noindent \textbf{Weight Sharing.} Below, we investigate weight sharing between the encoder-decoder pairs of all levels of our network to reduce the number of parameters in our model. Table \ref{tabel:share_weight} shows that weight sharing results in a slight loss of performance but reduces the number of parameters significantly.%, its runtime and running GPU memory remain at the same level.

%To conclude, our proposed DMPHN outperforms all recent deep image deblurring models on not only PSNR and SSIM, but also model size and runtime in case that we do not employ any recurrent network cells, e. g. LSTM, RNN and ConvLSTM. These results verify the effectiveness of capturing non-uniform motion blurs from multi-patch hierarchy.

\begin{figure}[htp]
    \vspace{-0.3cm}
    \centering
    \includegraphics[height=4.5cm]{images/saliency_comp.png}
    \caption{Instances of saliency detection on MSRA-B dataset.}
    \label{fig:saliency_comp}
    \vspace{-0.3cm}
\end{figure}

\begin{figure*}[htp]
	\centering
	\includegraphics[width=\linewidth]{images/Comp2}
	\caption{\small The instances of deblurred images. The first column contains the original blurred images, the second column uses \cite{nah2017deep}, the third column uses \cite{tao2018scale}. Finally, the last column presents our results. As can be seen, our model achieves the best performance across different scenes.}
	\label{fig:Comp2}
\end{figure*}

%===========================================================
\subsection{Saliency Prediction Extension}
We perform saliency detection with our proposed model to investigate the generalization ability on different tasks. Our proposed model is evaluated on MSRA-B dataset. This dataset consists of 3000 images for training and 2000 images for testing. Note that all current deep methods of saliency detection highly depend on VGG or ResNet pre-trained on ImageNet and these methods even cannot converge without the prior knowledge learned from ImageNet. By contrast, our network can be easily trained from scratch and outperforms all conventional methods. We evaluated single VMPHN for quantitative analysis. To make our network compatible with saliency detection task, the output channel is modified to 1 for gray image generation, and the residual connection between input and output at level 1 is disabled in VMPHN.

\begin{table}[h]
\makebox{\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\small{Models} & DRFI & RBD & DSR & MC & HS & OURS \\ \hline
$F_{\beta}$ & .7282 & .7508 & .7227 & .7165 & .7129 & .7682\\
\small{MAE} & .1229 & .1171 & .1207 & .1441 & .1609 & .1072\\ \hline
\end{tabular}}
\caption{\small Quantitative analysis of saliency detection on MSRA-B dataset \cite{nah2017deep}. $F_{\beta}$ is higher better, and MAE is lower better.}
\label{tabel:share_weight}
\vspace{-0.4cm}
\end{table}



==> introduction.tex <==
\section{Introduction}
The goal of non-uniform blind image deblurring is to remove the undesired effects of blur caused by the camera motion and the scene dynamics. 
Prior to the deep learning methods, conventional image deblurring methods employed variety of constraints/regularizations to approximate the kernel of motion blur or the scene dynamic, which generally require an expensive optimization. Moreover, the simplistic spatially-uniform motion blur kernel assumption makes such methods fail to remove complex patterns of blur in real world challenging scenarios.

\begin{figure}[htp]
%\vspace{-0.5cm}
	\centering
	\includegraphics[height=5cm]{images/PRPlot}
	\caption{\small The PSNR VS run time of state-of-the-art deep learning based motion deblurring methods and our proposed method on the GoPro dataset \cite{nah2017deep}. The blue region denotes real time inference, while the red region represents high performance motion deblurring. Clearly, our method achieves the best performance at 30 fps for $1280\times 720$ images, which is 40$\times$ faster than the very recent method \cite{tao2018scale}. A stackable version of our model further improves the performance with the cost increasing run time.}
	\label{fig:PRPlot}
%    \vspace{-0.5cm}
\end{figure}
\begin{figure*}[htp]
\vspace{-0.6cm}
	\centering
	\includegraphics[width=\linewidth]{images/DMPHN}
	\caption{\small Our proposed deep multi-patch hierarchical network (DMPHN). Note that our sliced patches have no overlapping between each other so they will cause boundaries in the output. However, these boundaries can be repaired by the process of upper level.}
	\label{fig:DMPHN}
    \vspace{-0.3cm}
\end{figure*}
\iffalse
\begin{figure*}[htp]
\vspace{-0.6cm}
	\centering
	\includegraphics[width=\linewidth]{images/Structure_Comp}
	\caption{\small Comparison between different network structures such as (a) \cite{nah2017deep}, (b) \cite{tao2018scale} and (c) ours. Our network does not employ any skip, upsample or recurrent connections. Best viewed on screen in color.}
	\label{fig:Structure_Comp}
    \vspace{-0.3cm}
\end{figure*}
\fi
%Note that in our network, the direct connection denotes a sum up operation between {\color{blue} on source and target.}

The success of Convolutional Neural Networks (CNN) \cite{krizhevsky2012imagenet,simonyan2014very} in high-level vision tasks motivated application of CNNs in low-level vision tasks such as image denoising \cite{} and deblurring \cite{}. Nah \etal \cite{nah2017deep} demonstrated the ability of CNN models in removing motion blur from multi-scale blurry images. Following this work, very recently, Tao \etal \cite{tao2018scale} proposed a highly effective scale-recurrent network for deblurring. However, it can be seen that multi-scale or scale-recurrent network architectures result in expensive run time as illustrated in Fig.~\ref{fig:PRPlot} with very limited benifits from multi-scale design. Furthermore, \cite{nah2017deep} pointed out that the increasing network depth with very lower resolution input in multi-scale approach are not helpful in deblurring. 

In contrast to the multi-scale and scale-recurrent architectures, our multi-patch model captures rich local information at the original resolution. Note that aggregating over multiple patches has been widely used in image classification \cite{lazebnik2006beyond,he2014spatial,lu2015deep,koniusz2018deeper}. For example, \cite{lazebnik2006beyond} proposes the Spatial Pyramid Matching (SPM) which divides images into coarse-to-fine grids in which histograms of features are computed. In \cite{koniusz2018deeper}, a second-order fine-grained image classification model uses overlapping patches for aggregation. 
In \cite{sun2015learning}, CNN estimates the motion blur kernel at the patch-level. With overlapping 30$\times$30 patches, they predict the probabilistic distribution of the blur kernels. However, their restoration model uses the conventional energy optimization.

In this paper, in contrast to the above multi-scale and scale-recurrent architectures, we propose a high-performance motion deblurring approach which leverages the local patch information. Specifically, we propose a simple and effective multi-level CNN model called Deep Multi-Patch Hierarchical Network (DMPHN) which uses multi-patch hierarchy as input. In this way, both the local and global information is effectively integrated. Our experiments verify the effectiveness of our locality-based model and demonstrate clear benefits of using the multi-patch hierarchy for motion deblurring. To the best of our knowledge, we are the first to propose a multi-level CNN approach to removal of the motion blur. Moreover, DMPHN is the first model which supports deblurring of 720p images real-time (runs at 30fps). 

In addition, 'depth-barrier' has been observed on both multi-scale and multi-patch model, which means increasing model depth by introducing very lower resolution or very finer segmentation can not improve the overall performance effectively. To address this problem, we present two upgraded stacking networks, whose performance achieved in this paper is way better than previous state-of-the-art.  
%
Our  contributions are summarized below:
\begin{itemize}
\item We propose an end-to-end CNN hierarchical model that exploits the local information that helps remove the motion blur and restore sharp images. Each finer level acts in residual manner by contributing its residual image to the coarser level (one level up).
\item We introduce novel stacking methods to effectively solve the 'depth-barrier' problem of current deep deblurring model.
\item We perform the baseline comparison (sanity check) to verify the difference between multi-scale and multi-patch approaches in the common testbed (for fair comparison).
\item We investigate the influence of sharing weights between the encoder-decoder pairs of different levels, and we propose a memory-friendly modification of DMPHN.
%\item Our framework could run in real time in dealing with 720p images.
%{\color{red}{Not a contribution ... this is the outcome of your contributions! It is like claiming that obtaining 99\% accuracy is a contribution ...}}
\end{itemize}

==> related.tex <==
\vspace{-0.5cm}
\section{Related Work}
%\YD{The related work seems not very extensive. Let's try to cover more recent work and do not miss some. How about the GAN based recent work.}
%In this section, we briefly review related work in image deblurring, which can be roughly classified as conventional methods methods and deep learning based methods.

Conventional image deblurring methods \cite{cho2009fast,jia2007single,xu2010two,levin2007blind,rajagopalan2014motion,jia2014mathematical,hyun2015generalized,sellent2016stereo} fail to remove realistic non-uniform motion blur because of their use of the spatially-invariant kernel. Moreover, their complex computational model leads to a long processing time, which cannot satisfy the growing needs for real-time processing.

%\cite{hyun2015generalized} proposed pixel-wise kernel with bidirectional optical flows to handle locally varying and general blurs caused by various sources, such as camera shake, moving objects. They used a single energy model that simultaneously estimates optical flows and latent frames to solve deblur problem. 

%\cite{sellent2016stereo} proposed to use stereo video to aid the challenging video deblurring task. They leverage 3D scene flow to induce accurate blur kernels via local homographies.

%\cite{pan2017simultaneous} presented a method to exploit the piece-wise planar assumption about the scene. Unlike previous video deblurring works, they used a single framework to jointly estimate the scene flow and deblur the image.

\noindent\textbf{Deep Deblurring.} Recently, CNNs have been applied to the problem of non-uniform image deblurring to deal with a complex motion blur in the time-efficient manner \cite{xu2014deep,sun2015learning,nah2017deep,schuler2016learning,nimisha2017blur,su2017deep,zhang2018adversarial}.
Xu \etal \cite{xu2014deep} proposed a deconvolutional CNN which removes blur in non-blind setting by recovering a sharp image given the estimated blur kernel. Their network uses separable kernels which can be decomposed into a small set of filters.  
Sun \etal \cite{sun2015learning} estimates and removes a non-uniform motion blur from an image by learning regression between 30$\times$30 image patches and their corresponding kernels. Subsequently, they employ the conventional optimization to estimate the latent image. % given the regressed local kernel and blurred image.
Su \etal \cite{su2017deep} presents a deep learning frameworks to process blurry video sequences and accumulate information across frames. This method does not require all pairs of samples to be aligned spatially.
Nah \etal \cite{nah2017deep} exploits a multi-scale CNN to restore sharp images in an end-to-end fashion from images whose blur is caused by various factors. A multi-scale loss function is employed to mimic the coarse-to-fine pipeline in conventional deblurring approaches.

%A method \cite{Vasu_2018_CVPR} leverages CNNs to deal with kernel uncertainty {\color{red}what is kernel uncertainty?} in non-blind image deblurring {\color{red}I may miss some knowledge here: what is non-blind deblurring?}. They used images obtained from non-blind deblurring scheme corresponding to different prior strengths of blur as input to train CNNs. 

Recurrent Neural Network (RNN) is a popular tool employed recently in deblurring  due to its advantage of processing information sequentially. A network consisting of three deep CNNs and one RNN, proposed by \cite{zhang2018dynamic}, is a prominent example. The RNN is applied as a deconvolutional decoder on feature maps extracted by the first CNN module. Another CNN module learns weights for each layer of RNN. The last CNN module reconstructs the sharp image from deblurred feature maps. Scale-Recurrent Network (SRN-DeblurNet) approach \cite{tao2018scale} uses ConvLSTM cells to aggregate the feature maps from coarse-to-fine scales. This shows the advantage of RNN units in non-uniform image deblurring task.

Generative adversarial nets (GAN) have also been employed in deblurring task due to its advantage on preserving texture details in images and generating solutions that are more close to real image. Kupyn \etal \cite{kupyn2017deblurgan} presented a conditional GAN network, which can produce high-quality delburred image with the Wasserstein loss constraints.

